Interpretable Prediction of Pulmonary Hypertension in Newborns using Echocardiograms

Pulmonary hypertension (PH) in newborns and infants is a complex condition associated with several pulmonary, cardiac, and systemic diseases contributing to morbidity and mortality. Therefore, accurate and early detection of PH is crucial for successful management. Using echocardiography, the primary diagnostic tool in pediatrics, human assessment is both time-consuming and expertise-demanding, raising the need for an automated approach. In this work, we present an interpretable multi-view video-based deep learning approach to predict PH for a cohort of 194 newborns using echocardiograms. We use spatio-temporal convolutional architectures for the prediction of PH from each view, and aggregate the predictions of the different views using majority voting. To the best of our knowledge, this is the first work for an automated assessment of PH in newborns using echocardiograms. Our results show a mean F1-score of 0.84 for severity prediction and 0.92 for binary detection using 10-fold cross-validation. We complement our predictions with saliency maps and show that the learned model focuses on clinically relevant cardiac structures, motivating its usage in clinical practice.

==> tex/questions.tex <==
1. How did the doctor came up with the diagnosis, i.e. did he measure some indices like chamber volumes, strain, etc... or did he just look at the video? + if they know the inter-observer variability
2. Renamed KAPAP => PSAX, CV => A4C, LA => PLAX acc. to what seems to be mostly used in the literature. However, we don’t know what KAAP and KAKL are ? These are some short-axis views, and according to the literature these all seem to be called PSAX, but the at different ‘levels’. (Like our “KAPAP” is the PSAX  at the level of papillary muscles, then we have different versions of PSAX).
3. Machine / US probe details that was used to acquire the sequences. 
4. Ethics approval necessary for the data acquisition?
5. Read over introduction and dataset.

==> tex/results_table.tex <==
\begin{table}[b!]
\caption{Results for (a) PH severity classification and (b) binary PH  detection using spatio-temporal approach. \textit{MV-3} refers to majority voting of A4C, PLAX, and PSAX-P views. \textit{MV-All} refers to majority voting of all five views.}
\label{tab:experiment_res}
\centering
\begin{tabular}{ l | c | c | c | c | c | c}
\multicolumn{7}{c}{(a)}\\ \hline
 Views & AUROC & F1-Score & Precision & Recall & \makecell{Balanced\\Accuracy} & Confidence \\  \hline
 A4C & 0.77$\pm 0.03$ & 0.72$\pm 0.05$ & 0.75$\pm 0.05$ & 0.72$\pm 0.05$ & 0.65$\pm 0.06$ & 0.88$\pm 0.02$  \\ \hline
PLAX & 0.85$\pm 0.04$ & 0.78$\pm 0.05$ & 0.82$\pm 0.06$ & 0.79$\pm 0.06$ & 0.72$\pm 0.05$ & 0.89$\pm 0.03$ \\ \hline
PSAX-P & 0.85$\pm 0.04$ & 0.81$\pm 0.05$ & 0.83$\pm 0.06$ & 0.82$\pm 0.04$ & 0.73$\pm 0.06$ & 0.90$\pm 0.03$  \\ \hline

 \makecell[l]{MV-3} & 0.84$\pm 0.08$ & 0.83$\pm 0.05$ & 0.86$\pm 0.04$ & 0.83$\pm 0.05$ & 0.76$\pm 0.07$ & 0.91$\pm 0.02$ \\ \hline
 \makecell[l]{\textbf{MV-All}} & \textbf{0.86}$\mathbf{\pm 0.09}$ & \textbf{0.84}$\mathbf{\pm 0.06}$ & \textbf{0.86}$\mathbf{\pm 0.05}$ & \textbf{0.85}$\mathbf{\pm 0.05}$ & \textbf{0.78}$\mathbf{\pm 0.07}$ & \textbf{0.90}$\mathbf{\pm 0.02}$ \\ \hline
  \multicolumn{7}{c}{}\\
 \multicolumn{7}{c}{(b)}\\
 \hline
 Views & AUROC & F1-Score & Precision & Recall & \makecell{Balanced\\Accuracy} & Confidence \\  \hline
 $\textrm{A4C}^{*}$ & 0.83$\pm 0.05$ & 0.81$\pm 0.04$ & 0.84$\pm 0.03$ & 0.81$\pm 0.04$ & 0.81$\pm 0.04$ & 0.91$\pm 0.03$ \\ \hline
PLAX & 0.90$\pm 0.07$& 0.86$\pm 0.09$& 0.88$\pm 0.07$& 0.86$\pm 0.09$& 0.86$\pm 0.08$& 0.91$\pm 0.02$ \\ \hline
\textbf{PSAX-P} & \textbf{0.95}$\mathbf{\pm 0.04}$ & \textbf{0.92}$\mathbf{\pm 0.03}$ & \textbf{0.93}$\mathbf{\pm 0.03}$& \textbf{0.92}$\mathbf{\pm 0.03}$ & \textbf{0.94}$\mathbf{\pm 0.03}$ & \textbf{0.90}$\mathbf{\pm 0.03}$ \\ \hline

 \makecell[l]{MV-3} & 0.90$\pm 0.03$& 0.87$\pm 0.04$& 0.88$\pm 0.03$& 0.87$\pm 0.04$& 0.87$\pm 0.04$& 0.92$\pm 0.01$ \\ \hline
 \makecell[l]{MV-All} & 0.90$\pm 0.03$ & 0.89$\pm 0.02$ & 0.90$\pm 0.02 $& 0.89$\pm 0.02$ & 0.89$\pm 0.02$ & 0.91$\pm 0.01$ \\ \hline
\end{tabular}
\end{table}
